Token Merging via Spatiotemporal Information Mining for Surgical Video Understanding

Vision Transformer models have shown impressive effectiveness in the surgical video understanding tasks through long-range dependency modeling. However, current methods suffer from prohibitive computational costs due to processing massive spatiotemporal tokens across video frames. While prior work on token merging has advanced model efficiency, they fail to adequately consider the inherent spatiotemporal structure of video data and overlook the heterogeneous nature of information distribution, leading to suboptimal performance. In this paper, we propose a spatiotemporal information mining token merging (STIM-TM) method, representing the first dedicated approach for surgical video understanding. STIM-TM introduces a decoupled strategy that reduces token redundancy along temporal and spatial dimensions independently. Specifically, the temporal component merges spatially corresponding tokens from consecutive frames using saliency weighting, preserving critical sequential information and maintaining continuity. Meanwhile, the spatial component prioritizes merging static tokens through temporal stability analysis, protecting dynamic regions containing essential surgical information. Operating in a training-free manner, STIM-TM achieves significant efficiency gains with over $65\%$ GFLOPs reduction while preserving competitive accuracy across comprehensive surgical video tasks. Our method also supports efficient training of long-sequence surgical videos, addressing computational bottlenecks in surgical applications.

==> tables/foundation_model.tex <==
\begin{table}[t]
\aboverulesep=0ex
\belowrulesep=0ex
\setlength{\tabcolsep}{1pt} % Adjust the space between columns
\renewcommand{\arraystretch}{1.3}
\centering
\caption{
     Comparison of token merging methods on EndoFM-LV downstream tasks. Classification: Temporal (Blocks 1-6), Spatial (Blocks 7-12). Segmentation: Temporal (Blocks 1-3), Spatial (Blocks 4-12). GFLOPs and Memory are measured on the classification task.
}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c|c c|c|c|c}
\toprule
\multirow{2}{*}{$R_T$} & \multirow{2}{*}{$R_S$} & \multirow{2}{*}{GFLOPs$\downarrow$} & \multirow{2}{*}{Mem.(GB)$\downarrow$} & \multirow{2}{*}{Method} & \begin{tabular}[c]{@{}c@{}}PolypDiag\\ (classification)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CVC-12K\\ (segmentation)\end{tabular} \\ \cline{6-7} 
 &  &  &  &  & F1 Score$\uparrow$ & Dice$\uparrow$ \\ \midrule
 - & - & 786.82 & 7.48 & Baseline & 97.5 & 83.6 \\
 % \addlinespace[2pt]
\multirow{2}{*}{1} & \multirow{2}{*}{12} & 615.26 & 6.49 & ST-TESTA & 97.5 & 82.7 \\ 
 & & \cellcolor{highlight}615.21 & \cellcolor{highlight}6.78 & \cellcolor{highlight}STIM-TM & \cellcolor{highlight}97.5 & \cellcolor{highlight}83.5 \\ 
 % \addlinespace[2pt]
 \multirow{2}{*}{2} & \multirow{2}{*}{24} & 471.31 & 5.29 & ST-TESTA & 96.7 & 82.5 \\ 
 & & \cellcolor{highlight}471.28 & \cellcolor{highlight}5.74 & \cellcolor{highlight}STIM-TM & \cellcolor{highlight}97.5 & \cellcolor{highlight}82.8 \\ 
 \bottomrule
\end{tabular}
}
\label{tab:foundation}
\vspace{-10pt}
\end{table}

